Neural Parameter Allocation Search

Training neural networks requires increasing amounts of memory. Parameter sharing can reduce memory and communication costs, but existing methods assume networks have many identical layers and utilize hand-crafted sharing strategies that fail to generalize. We introduce Neural Parameter Allocation Search (NPAS), a novel task where the goal is to train a neural network given an arbitrary, fixed parameter budget. NPAS covers both low-budget regimes, which produce compact networks, as well as a novel high-budget regime, where additional capacity can be added to boost performance without increasing inference FLOPs. To address NPAS, we introduce Shapeshifter Networks (SSNs), which automatically learn where and how to share parameters in a network to support any parameter budget without requiring any changes to the architecture or loss function. NPAS and SSNs provide a complete framework for addressing generalized parameter sharing, and can also be combined with prior work for additional performance gains. We demonstrate the effectiveness of our approach using nine network architectures across four diverse tasks, including ImageNet classification and transformers.

==> 4_model.tex <==

\section{Shapeshifter Networks for NPAS}
\label{sec:ssn}

We now present Shapeshifter Networks (SSNs), a framework for addressing the NPAS task through generalized parameter sharing that learns to morph a fixed budget of parameters into the weights used by a neural network.  SSNs begin by learning the layers where parameter sharing is most effective in a short pretraining step (Section~\ref{subsec:mapping}), which we use to select the trainable parameters used to generate layer weights.  If the number of trainable parameters is greater than the number of layer weights, then we form them into templates and then learn a weighted linear combination of these templates to generate the layer's weights (Section~\ref{subsec:generation}). When the number of trainable parameters is less than the number of layer weights, then we provide an efficient method of upsampling the parameters (Section~\ref{subsec:upsample}).  Note that our approach does not require any changes to a model's loss function, architecture, or hyperparameters.  An overview of our SSNs is provided in Figure~\ref{}.

\subsection{Mapping layers to parameter groups}
\label{subsec:mapping}

Given layer $\ell_i$ and a set trainable parameters $\theta$ the first task is implement our function $\theta_i = f_{select}(\ell_i, \theta)$ to select a subset of parameters $\theta_i$ that we will use to generate the layer's weights $w_i$ (we will discuss weight generation in Section~\ref{subsec:generation}).  We note that $\theta_i$ may share some (or all) of its trainable parameters with other layers in a network, but sharing parameters between some layers may be more effective than others.  Thus, our first task is to learn a mapping of layers $\ell_{1,...,L}$ to $P$ parameter groups. We denote $\theta^j_i$ as the trainable parameters for layer $\ell_i$ which are selected from the $jth$ parameter group.
We treat the number of parameter groups as a hyperparameter (see supplementary for an ablation study on how the number of groups affects performance).  Prior work that shares parameters across layers can be thought of as using manual assignments of layers to parameter groups (\eg,~\citet{haHypernetworks2016,jaegle2021perceiver,savarese2018learning}), which are based on heuristics that don't generalize to many architectures as discussed in the Introduction.  In this paper, however, our goal is to automatically search for the optimal assignments without significantly increasing training time.

A simple brute force approach for mapping layers to parameter groups would be simply to try all possible permutations of assignments.  However, this would be infeasible for many tasks, as the size of the training data or the number of possible permutations would be very computationally expensive for a such an approach.  Instead, our approach finds layers whose weights can be generated effectively using the same parameters.  

We begin by reshaping the trainable parameters $\theta$ into $K$ evenly sized templates $T^{1,...K}$.  We note that each layer is a different size, so we perform bilinear interpolation to resize the templates are the same size as the weights $w_i$.  In other words, when we generate the weights for layer $\ell_i$, we ensure $\#params(w_i) = \#params(T_i^k)$ for all $T_i^k$. To encourage significant sharing between layers so that we can properly measure the effectiveness, we give a very small budget for the network in this pretraining step (\ie, we train a LB-NPAS model), regardless of the initial budget provided to the model. We found that a budget the same size of the weights of the largest layer in a network to work well.  We generate the weights for each layer using a weighted average of the templates, \ie,
\begin{equation}
    w_i = \sum_{k=1}^K \alpha_i^k T_i^k.
    \label{eq:weight_sum}
\end{equation}
Note that the coefficients $\alpha_i$ are either trainable parameters themselves (or generated from trainable parameters, see Section~\ref{subsec:generation} for more details).  These coefficients are learned end-to-end along with the trainable parameters $\theta$.  Thus, since the templates $T$ represent the same parameters across all layers, then layers with similar $\alpha_i$ result in weights that similar across layers.  Motivated by this intuition, we use k-means clustering over layer representations (like the coefficients $\alpha_{1...L}$) to separate layers into the $K$ parameter groups once our pretraining step is complete.  Layers in the same cluster get assigned to the same parameter group.  We set this pretraining step to account for increasing the total training time for a network by 10-15\%, which we found to be sufficient to determine which layers can effectively share parameter with each other.

\subsection{Implementing a network using a fixed parameter budget}
\label{subsec:implementation}

Mapping layers to parameter groups in Section~\ref{subsec:mapping} can be thought of as training a condensed version of a SSN model.  However, there are several modifications from the pretraining step we make once we have obtained this mapping.  First, now that we have the mapping of layers to parameters, we have to decide how to split them.  Distributing the parameters evenly among groups would likely be suboptimal, since the layers in each parameter groups may require different numbers of parameters.  Thus, we split the trainable parameters proportionally.  For example, if a layer accounts for 10\% of the total weights needed to implement a network architecture, then the parameter group it belongs to would get 10\% of the parameters in the budget.  We also do not automatically resize all parameter templates, and instead use only subsets of parameters for layers (unless too few are available).

More formally, given a mapping of layers $\ell_i$ to the $P$ parameter groups, we initialize a set of trainable parameters $\hat{\theta}^{1,...,P}$ equal to our parameter budget.  Remember that the number of trainable parameters varies across each parameter group proportionally to the number of weights required by its layers. We do not use any weights from the pretraining step in Section~\ref{subsec:mapping} due to the differences in the training procedures outlined above and the fact that the number of parameters used by the pretraining step is typically small, and may be less than the budget of our target network.  When doing a forward pass on the network we begin by selecting a subset of the trainable parameters $\hat{\theta}^j_i$ that we will use to generate each layer $\ell_i$.  There are three possible cases that we must consider, which we use to implement the weight generation funcion $w_i = f_{gen}(\ell_i, \hat{\theta}^j_i)$.  First, the number of trainable parameters $\hat{\theta}^j_i$ may be equal to the number of weights $w_i$ that are required by the operation being performed by layer $\ell_i$. In this case the layer will simply use the available parameters to perform its operation directly, \ie, we set $w_i = \hat{\theta}^j_i$.  Second, the number of trainable parameters may be greater than weights required by the layer.  In this case we learn a linear combination of templates like used Eq.~\ref{eq:weight_sum}, which we will discuss in more detail in Section~\ref{subsec:generation}.  Finally, the number of trainable parameters may be smaller than weights required by the layer.  Thus, in this case our trainable parameters requires upsampling, which we will discuss in Section~\ref{subsec:upsampling}.  Once we have generated the weights we perform its layer operation on the layer's input data and proceed to the next layer.

\subsubsection{Generating weights from templates}
\label{subsec:generation}

Given trainable parameters $\hat{\theta}^j_i$ the task is to generate the weights for layer $\ell_i$.  When a SSN uses this module to generate weights, we know that the number of parameters in $\hat{\theta}^j_i$ is greater than the number of desired output weights $w_i$.  We begin by reshaping the trainable parameters to produce up to $K$ \emph{templates} $\hat{T}_i^{1,...,K}$ so that they are the same dimensions as $w_i$.  Note that unlike our pretraining step described in Section~\ref{subsec:mapping}, we only reshape the trainable parameters into templates and do not resize them.  Formally, let $D^1_i, \ldots, D^M_i$ be the dimensions of $w_j$. We interpret $\theta_i^j$ as a vector and reshape it to have dimensions $\tilde{K}_i \times \min(\prod D_i^i, |\theta_i^j|)$, where we ignore excess parameters and $\tilde{P}_i = \max(1, \min(\lfloor |\theta_i^j| / \prod D_k^j \rfloor, K))$.  
%Each template is assigned as $T_i = \theta_i[k,:]$, $k = 1, \ldots, \tilde{P}$.
Hence, we produce at most $K$ full templates.  

If fewer than 2 templates can be created, we directly use the single template as the weights for the layer.  However, more than $K$ templates may be created from the trainable parameters $\hat{\theta}^j_i$. If we were to provide the first $K$ templates for each layer, then it could result in an uneven sharing of the available parameters.  For example,  say we set $K=1$ in a network that has three layers in the same parameter group, and two layers $\ell_1, \ell_2$ requires 100K weights, while the third layer $\ell_3$ requires 200K weights, then the first 100K parameters in $\hat{\theta}^j_i$ would be shared by all three layers, and the second 100K parameters would only be used by $\ell_3$.   Instead, we allocate parameters in a round robin fashion.  So if the number of trainable parameters in $\hat{\theta}^j_i$ is 200K, then $\ell_1$ would use the first 100K parameters and $\ell_2$ would use the next 100K parameters, with $\ell_2$ sharing half of its parameters with $\ell_1$ and the other half with $\ell_2$.  As a result, no portion of trainable parameters is shared with more than 2 layers.  Note that the number of templates $K$ is a hyperparameter, and we provide an ablation study of how it affects performance in the supplementary.

Given weight templates $\hat{T}_i^{1,...,K}$ we can generate layer weights by using a weighted combination of the templates as done in Eq.~\ref{eq:weight_sum}.  Making the coefficients $\alpha_i^k$ trainable parameters would follow the approach of \citet{savarese2018learning} for generating weights, which we shall refer to as \textbf{WAvg}.  While this provides an efficient mechanism for generating weights, similarities between layers are only learned implicitly.  Specifically, when we train a model during our pretraining step in Section~\ref{subsec:mapping}, we can infer that two layers are similar due to their $\alpha_i^k$ ending up in a similar to each other, but nothing in the model explicitly encourages this to occur. This means that it could be that a network gets stuck in a local minimum where two templates have similar representations since different layers put high weight on only one of the templates. Thus, we propose an approach for predicting each layer's $\alpha_i^k$ where each layer that has the same number of templates are predicted using a shared fully connected layer.

Formally, \textbf{Layer embeddings (Emb)} use a vector of trainable parameters $\phi_i$ to represent the layer. In our experiments we set the dimensions of $\phi_i$ to be 24, which we found to work well.  Then we use a shared linear layer across any layer within the same parameter group, which is parameterized by $W_e, b_e$, to predict the coefficients $\alpha_i$. \Ie, $\alpha^{'j} = W_e \phi_i + b_e$, which are used to generate weights using Eq.~\ref{eq:weight_sum}.  Note that we also attempted predict these coefficients using an MLP with more layers and nonlinearities, but it did not improve performance.  Although \emph{Emb} technically requires more trainable parameters than \emph{WAvg}, the differences are negligible.  For example, if the number of templates $K=8$, then using Emb would only result in $24 \times 8 + 8 = 232$ trainable parameters for the shared linear layer predicting the coefficients, and $24$ trainable parameters used for each layer.

During our pretraining step in Section~\ref{subsec:mapping} we experiment with using both \emph{WAvg} and \emph{Emb} weight generation methods.  In the final clustering step where we combine layers into parameter groups, we cluster based on  $\alpha_i$ for \emph{WAvg}, but use the layer embeddings $\phi_i$ for \emph{Emb}.   

\subsubsection{Upsampling Parameters}
\label{subsec:upsample}

If the number of parameters in $\hat{\theta}_i^j$ is less than the number of desired weights $w_i$ for some layer $\ell_i$, then there are not have sufficient parameters to implement the layer directly. We note that this is a challenge seen in NPAS that does not occur with other parameter sharing methods.
We address this with a \emph{parameter upsampler}, which upsamples the parameters $\hat{\theta}_i^j$ to the size needed by $w_j$.

A na\"{i}ve baseline is to use \textbf{bilinear interpolation (inter)} to upsample parameters.
However, this could alter the kinds of filter patterns the parameters would capture, as the parameters would effectively stretch a filter's receptive field.
In practice, we found that fully-connected and recurrent layers could compensate for this kind of warping.
Convolutional layers, in contrast, degrade in performance compared to simpler baselines, such as repeating parameters by tiling (see supplementary), as spatial information is more critical.

Since repeating parameters creates redundancies in weights, we propose a method that modifies parameters to capture new concepts using a learned \textbf{mask}.
The unmodified parameters are first used, and each subsequent repetition of the parameters is multiplied element-wise by a mask applied over windows of sequential parameters.
By default, the window is of size 9 (for the commonly-used $3 \times 3$ kernels in CNNs), which we found to work well, but any size can be used.
Even if several masks are required, the number of additional parameters is negligible.

For example, let us assume that $\hat{\theta}_i^j$ contains 1M parameters, but $w_i$ requires 3M weights.  In this case, we would use $(3\text{M} - 1\text{M}) / 1\text{M} = 2$ learned masks $\psi_1, \psi_2$, each of which are $N=9$ dimensional, to upsample the parameters by a 2M weights. Then, we perform an elementwise multiplication between windows of $\hat{\theta}_i^j$ and each $\psi_x$.  These parameter windows are generated using a sliding window approach with stride $N$. The result of this operation is the modified parameters $\hat{\theta}^j_{i, \psi_{1}}$ and $\hat{\theta}^j_{i, \psi_{2}}$.  Finally, we would concatenate together $\hat{\theta}_i^j$ with $\hat{\theta}^j_{i, \psi_{1}}$ and $\hat{\theta}^j_{i, \psi_{2}}$ to create $w_i$.  Note that these masks are shared between layers in the same parameter group, and we always give preference to using the original unmodified parameters.  As such, for another layer needing 1.5M weights from the same parameter group would end up concatenating together $\hat{\theta}_i^j$ with half of $\hat{\theta}^j_{i, \psi_{1}}$ to generate them. 


%\subsection{Comparison to closely related work}
%\label{subsec:comparison}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/filter_example.pdf}
    \caption{The local filter patterns required by many layers in a neural network may be generated using a low-rank representation and linearly combined.  A key observation of this work is that these filter patterns can also generalize across layers of different sizes or performing different operations (\ie, some local patterns may be useful for both fully connected and convolutional layers).  Our NPAS approach automatically learns where these repeated patterns exist in a neural network across all layers, regardless of size or type, creating an efficient and effective representation.}
    \label{fig:filters}
\end{figure}

%At a high level, our SSNs learn how to generate the weights of a network as opposed to optimizing layer weights themselves.  Closest to our work is \citet{savarese2018learning}, who introduced a cross-layer parameter sharing method that learned how to mix templates of convolutional layer weights in order to more effectively use the available parameters by learning a set of basis filters and linearly combining them.  Hypernetworks~\citep{haHypernetworks2016} use an multilayer perception (MLP) to directly predict a layer's weights.  While these might seem variations on a similar theme at first glance, they have significant differences in practice.  For example, when reusing parameters many times to generate weights for many layers all the weights generated by Hypernetworks would be the same for each layer.  Creating a new MLP to generate different weights is possible, it would be far more expensive than simply using new mixing parameters for the templates to generate unique weights for each layer. Our SSNs also rely on template mixing, but \citet{savarese2018learning} only learns to share parameters between identical layers using hand-crafted strategies that means it cannot generalize to architectures like DenseNets, whereas our SSNs are automatic and generalize to any architecture.

%Another key benefit of our SSNs when addressing the LB-NPAS setting, where we reduce parameters used to represent a network, is that they can be used to reduce memory and communications costs during training.  Low-rank decomposition methods also reduce the number of parameters in a network, but often require training the full-rank model first (\eg,~\citet{frankle2018lottery,lee2019snip}), so they do not reduce memory requirements during training.  In addition, these methods do not generalize well across different layer types~\citep{Zhang2020OneShot}, whereas our SSNs can be applied to any architecture.  Although substantial memory requirements also arise for storing activations, this can be substantially reduced by leveraging gradient checkpointing techniques (\eg,~\citet{Chen2016TrainingDN,gomezReversible2017,jain2019checkmate}).  Thus, many neural networks leverage cross-layer parameter sharing to reduce the size of their model and help prevent overfitting (\eg,~\citet{dehghani2018universal,jaegle2021perceiver}). However, these methods require many identical layers in a network to be effective.  Specifically, they can only reduce the size of $\theta$ by a factor of the number of identical layers in the network.  For example, a 100M parameter network with three identical layers with 1M parameters can only reduce memory by $(3 - 1) \times 1\mathrm{M} = 2/100\mathrm{M}$ parameters, greatly minimizing the potential benefits of prior work.  In contrast, our SSNs can implement any architecture with any parameter budget, \ie, they can be used to implement the three 1M parameter layers while using only 0.1M parameters.

%%% Local Variables:
%%% TeX-master: "0_main"
%%% End:


\section{Shapeshifter Networks for NPAS}
\label{sec:ssn}


By combining gradient checkpointing techniques that reduce memory from activations  with prior work in cross-layer parameter sharing   with . While one could manually implement a method of offloading model weights rather than sharing parameters between layers (\eg, out-of-core, Unified Memory, pipeline/model-parallelism), it is complex and involves tradeoffs (\eg, slow off-GPU communication). SSNs materialize weights for a layer on-demand, \emph{without} off-chip communication to slower (\eg, DRAM, remote) memory and with low overhead.

We now present Shapeshifter Networks (SSNs), which solve the NPAS task by automatically learning where and how to share parameters in a network.
By learning to combine a set of bases to create the patterns required by layers (Figure~\ref{fig:filters}), we can obtain a more efficient parameter representation.  Prior work used hand-crafted heuristics that learned this decomposition for identical layers~\cite{bai2019deep,dehghani2018universal,Lan2020ALBERT,savarese2018learning}, which makes them ill-suited for NPAS (Section~\ref{subsec:challenges}). 

An SSN consists of one or more \emph{parameter stores} $S_i = (\theta_i, \ell_i)$, where $\theta_i \subseteq \theta$ is a set of parameters for use by the store and $\ell_i \subseteq f_{\{1, \ldots, L\}}$ is the set of layers associated with that store, which may share parameters.
The $\theta_i$ and $\ell_i$ partition the parameters and layers (resp.) so each parameter and layer is associated with exactly one store.
In addition, a parameter store has a \emph{parameter selector} (Section~\ref{subsec:selector}), a \emph{weight generator} (Section~\ref{subsec:generation}), and, if necessary, a \emph{parameter upsampler} (Section~\ref{subsec:upsample}).
We begin by assuming the mapping from layers to parameter stores is provided; we discuss learning these in Section~\ref{subsec:param-mapping}.
Finally, we present here methods that are broadly successful for SSNs.
The supplementary contains discussion of additional methods, comparisons, and ablations.

%In contrast, our Shapeshifter Networks (SSNs), automatically learns to where and how to share parameters in a network.  Essentially, our SSNs can take any number of parameters and morph them to fit the weights desired by a network architecture.  There are two problems that we have to address to accomplish this feat effectively, which have not been investigated in prior work.  First, we learn how to automatically identify the layers where parameter sharing is effective (Section~\ref{subsec:selector}). Second, we learn to generate weights, even when layers request more parameters than are available (Section~\ref{subsec:generation}).

%We now describe Shapeshifter Networks in detail. 
%
%A simple feed-forward network like those in Figure~\ref{fig:parameter_sharing} can be thought of as applying $L$ layer operations $f_{\{1,...,L\}}$ to input data $x$ given model parameters $\theta$. For simplicity, we present this case and also neglect layers that do not require parameters, but our approach is applicable to any architecture.  
%\htor{this sounds limiting, it would also work for recurrent or skip conns, no?}
%
%For simplicity, we ignore layers that do not require model parameters like activation functions. 
%
%A traditional neural network would implicitly choose the layer parameters for each learnable operation $f_i$.
%
%In contrast, SSNs decouple the $f_i$ from their parameters, and instead query a parameter store (Section~\ref{subsec:allocator}) to obtain weights to perform its operation.  Parameters from regularization layers such as Batch Normalization~\cite{IoffeBatchNorm2015} are not shared with other layers.  We note these layers typically have a negligible contribution to the number of parameters in a neural network, but all other operations requiring parameters may end up sharing weights.  Some layers may require a parameter store to perform weight upsampling (Section~\ref{subsec:upsample}) when it needs more weights than are available. In addition, some layers may find sharing parameters detrimental to performance, and so we learn to split layers into parameter groups (Section~\ref{subsec:groups}).  Each group has its own parameter store (\ie, parameters are not shared between groups).   SSNs do not require modifying a network's architecture or its loss function, making them easy to adapt to any task or network.
%
%SSNs make no prior assumptions about a model's architecture, so they can be used to implement any neural network with arbitrary numbers of parameters.


%A traditional neural network could be implemented using our framework by placing each layer in its own parameter group and then allocate the minimum number of parameters required to implement each operation.  However, a Shapeshifter network need not be contrained in such a manner, layers may

\subsection{Selecting Parameters from a Parameter Store}
\label{subsec:selector}

A \emph{parameter selector} for a parameter store $S_i$ selects a subset of the store's parameters $\theta_i$ that will be used to generate the weights of each layer $f_j \in \ell_i$ associated with the store.
The selector does this by producing up to $P$ (a hyperparameter) \emph{templates} $T_1^j, \ldots, T_P^j$ for each $f_j$, which are used by the parameter generator to produce the layer's weights $w_j$.
We do this as follows.
Let $D_1^j, \ldots, D_M^j$ be the dimensions of $w_j$. We interpret $\theta_i$ as a vector and reshape it to have dimensions $\tilde{P}_j \times \min(\prod D_k^j, |\theta_i|)$, where we ignore excess parameters and $\tilde{P}_j = \max(1, \min(\lfloor |\theta_i| / \prod D_k^j \rfloor, P))$.
Each template is assigned as $T_k^j = \theta_i[k,:]$, $k = 1, \ldots, \tilde{P}$.
Hence, we produce at most $P$ full templates, and at least one template; if too few parameters are available for a single full template, parameter upsampling will be used.
When more than $P$ templates can be produced, parameters are allocated to layer templates in a round robin fashion.

%In a SSN all trainable parameters are managed by a parameter store.  Given a network architecture, the parameter store's job is to select the parameters that are used by each layer to generate its weights.  More formally, a parameter store has a set of trainable parameters $\psi_i \in \Psi$ used to generate weights for layers.  Each element $\psi_i$ represents a vector of parameters, and any layers that are associated with the same $\psi_i$ may share parameters. Let $D_1^j, \ldots, D_M^j$ be the dimensions of the parameters $\theta_j$ needed by a network architecture's $j$th layer. We obtain a candidate set of $P$ templates for layer $j$, $C_j \in \mathbb{R}^{P, D_1^j, ..., D_M^j}$, by reshaping its $\psi_i$ (ignoring excess).  If too few parameters are available for a single candidate, we use parameter upsampling (Section~\ref{subsec:upsample}).  Note that we may provide $P$ as a hyperparameter, which may be smaller than the number of candidates that can be constructed from $\psi_i$.  In this case, we allocate candidates in a round robin fashion to construct $C_j$.  Once we have selected the candidates for a layer, we learn a weighted combination of them to generate its weights (described in Section~\ref{subsec:generation}).

\subsection{Generating Weights from Templates}
\label{subsec:generation}

The \emph{weight generator} uses the selected templates $T_k^j$ for a layer $f_j$ to produce its weights $w_j$.
If there is only one template, it is used directly if there are sufficient parameters, and upsampled if not (Section~\ref{subsec:upsample}).
Otherwise, the weight generator uses a learned combination of the $T_k^j$ to generate $w_j$.
Combining templates allows an SSN to learn to combine basis filters (Figure~\ref{fig:filters}) or to \emph{not} share certain parameters.

We consider two methods for learning this combination (see the supplementary for discussion of additional methods).
These both use learned coefficients $\alpha^j$ for each layer, and the goal is to use a soft-attention mechanism~\cite{bahdanau2015neural} over the $T_k^j$ to obtain $w_j$.
The $\alpha^j$ are initialized orthogonally to the coefficients of each other layer in the store, so that the features are as far from other layers' features as possible.
The number of additional parameters used is negligible.
\smallskip

\noindent\textbf{Template weighted averaging (WAvg)} uses a weighted average over templates to generate $w_j$, and was introduced by Savarese~\etal~\cite{savarese2018learning}.
The coefficients $\alpha^j$ are of size $\tilde{P}_j$ and are directly learned for each layer.
The model weights are computed as a weighted average:
\begin{equation}
    w_j = \sum_{k=1}^{\tilde{P}_j} \alpha_k^j T_k^j.
    \label{eq:weight_sum}
\end{equation}

\noindent\textbf{Layer embeddings (Emb)} use the $\alpha^j$ to represent the layer in a learned embedding.
The coefficients $\alpha^j$ are of size $\tilde{P}_j \times 24$ (where $24$ is a hyperparameter we found to work well).
An embedding $E_j$ produces $\tilde{P}_j$ output coefficients $\alpha^{'j} = \mathrm{softmax}(E_j(\alpha^j))$ which are used in a weighted average (replacing the $\alpha^j$ in WAvg).
The embedding $E_j$ is shared between all layers in the parameter store that select from the same set of templates, which enables us to identify when layers can be implemented using similar parameters.

To implement $E_j$, we found that a simple fully-connected layer with weights $W_j \in \mathbb{R}^{24 \times \tilde{P}_j}$ and bias $b_j \in \mathbb{R}^{\tilde{P}_j}$ works well; using an MLP with more layers and nonlinearities did not improve performance.

%Once we obtain the candidates $C_j$ from the parameter selection process in Section~\ref{subsec:selector}, we most learn how to combine them to generate a layer's weights.  If $|C_j| > 1$, we generate weights using a weighted combination of the candidates (Section~\ref{subsubsec:learned_allocation}).  If $|C_j| = 1$, then we can directly use the candidate if it has sufficient parameters for a layer.  Otherwise, if it needs additional parameters we upsample them using the process in Section~\ref{subsec:upsample}.

%\subsubsection{Learned Candidate Combination}
%\label{subsubsec:learned_allocation}

%We now describe strategies that use learned coefficients $\alpha_j$ to combine the candidates in set $C_j$.
%
%Essentially, the goal is to use a soft-attention mechanism~\cite{bahdanau2015neural} over $C$ to obtain the layer parameters. Each strategy begins with features $\phi_i$ representing each layer $i$. These features use an orthogonal initialization so that they begin as far from other layers' features as possible. In this paper we explore two methods of learning $\alpha_j$, which are described below. 
%\smallskip
%
%\noindent\textbf{Candidate weighted averaging (WAvg)} uses a weighted average over available candidates, and was introduced by Savarese~\etal~\cite{savarese2018learning}.  The coefficients used to combine the candidates are directly learned for each layer. 
%Then, the model weights are computed via:
%\begin{equation}
%    \theta_j = \sum_{k=1}^{|C_j|} \alpha_{jk} C_{jk}
%    \label{eq:weight_sum}
%\end{equation}
%where $\theta_j$ is the weighted sum of each candidate.
%\smallskip

%\noindent\textbf{Layer embeddings (Emb)} represent each layer by an embedding $\phi_i$ resulting in a $L \times |C_j| \times 24$ feature tensor.  From these embeddings we predict the coefficients $\alpha$ for combing the candidates using Eq.~(\ref{eq:weight_sum}) using a fully connected (FC) layer. Layers that operate over the same set of candidates use the same FC layer, which enables us to identify when layers can be implemented using similar parameters as their embeddings will end up near each other.  We did try to use a MLP with more layers and nonlinear activation functions, but it did not improve performance.  More formally, let $W_p$ and $b_p$ be the weights and bias of a FC layer with output dimension $|C_j|$. Then we obtain coefficients with:
%\begin{equation}
%    \alpha_j = \mathrm{softmax}(\phi_iW_p + b_p).
%    \label{eq:emb_attention}
%\end{equation}
%\htor{unclear, maybe specify exact tensor contraction that implements the embedding (at least in supp)?}

\subsection{Upsampling Parameters}
\label{subsec:upsample}

If $|\theta_i| < |w_j|$ for some layer $f_j$ in parameter store $S_i$, then the store does not have sufficient parameters to implement the layer directly.
This is a challenge seen in NPAS that does not occur with other parameter sharing methods.
We address this with a \emph{parameter upsampler}, which upsamples the parameters $\theta_i$ to the size needed by $w_j$.

A na\"{i}ve baseline is to use \textbf{bilinear interpolation (inter)} to upsample parameters.
However, this could alter the kinds of filter patterns the parameters would capture, as the parameters would effectively stretch a filter's receptive field.
In practice, we found that fully-connected and recurrent layers could compensate for this kind of warping.
Convolutional layers, in contrast, degrade in performance compared to simpler baselines, such as repeating parameters by tiling (see supplementary), as spatial information is more critical.

Since repeating parameters creates redundancies in weights, we propose a method that modifies parameters to capture new concepts using a learned \textbf{mask}.
The unmodified parameters are first used, and each subsequent repetition of the parameters is multiplied element-wise by a mask applied over windows of sequential parameters.
By default, the window is of size 9 (for the commonly-used $3 \times 3$ kernels in CNNs), which we found to work well, but any size can be used.
Even if several masks are required, the number of additional parameters is negligible.


%One of the new challenges addressed in this work is how to effectively upsample weights when a layer requests more parameters than are available in a store.  A naive approach would be simply use \textbf{bilinear interpolation (inter)}.  However, this could alter the kinds of local filter patterns the parameters would capture, as upsampling these parameters would effectively stretch a local pattern's receptive field.  In practice, we found that fully connected and recurrent layers could more easily compensate for this kind of warping.  However, convolutional layers, where spatial information is more critical, performance would often degrade compared with simpler methods such as just repeating the parameters. For example, if a FC layer asks for a $100 \times 100$ weight matrix, but the largest weight matrix the store can make is $50 \times 100$, one could simply make a copy and concatenate them together.  {\color{red} should make a bolded reference to mask in this section}

%Since repeating parameters creates redundancies in the weights, we also propose a method that learns how to modify the parameters to capture new concepts.  These modifications come in the form of a learned mask that are multiplied element-wise over windows of parameters (\ie, sets of sequential parameters). By default, we group parameters in windows of size 9 (for the commonly-used $3 \times 3$ kernels in CNNs), which we found to work well, but any size can be used. Even if several masks are required to learn multiple alterations of parameters, only a negligible number of learned parameters are required.  

\subsection{Learning Parameter Store Mappings}
\label{subsec:param-mapping}

Finally, layers must be assigned to parameter stores.
We will treat the number of parameter stores used by the SSN as a hyperparameter.
While layers could be manually assigned to stores (as done in prior work), we instead present an approach to automatically group layers where parameter sharing is most effective.
Our approach is guided by the hypothesis that if two layers learn similar coefficients over the same set of templates in their weight generator, the generated weights will be similar and the layers can share parameters with little (or no) performance degradation.

We begin by assigning all layers and parameters to a single parameter store and then perform a short pretraining stage lasting for a small number of epochs.
To ensure each layer operates on the same set of templates, we split the parameters into equal-sized templates $T_1^j, \ldots, T_C^j$ (we found $C = 4$ worked well).
Each template $T_k^j$ is then resized to be the same size as the layer's weights $w_j$.
This may involve up- or downsampling of parameters, and we therefore use inter up/downsampling for this stage.
Finally, the templates are used by a weight generator to generate $w_j$.
When pretraining completes, we perform $k$-means clustering on the layer coefficients $\alpha^j$, with one cluster for each store desired.
Each store $P_i$ is then allocated parameters $\theta_i \subseteq \theta$, where $|\theta_i|$ is proportional to the size of the required weights in that store (\ie, $|\theta_i| = (\sum_{j \in \ell_i} |w_j| / \sum_{j \in \{1, \ldots, L\}} |w_j|) |\theta|$).

Standard training then proceeds from scratch with the learned stores.
Note we cannot reuse the parameters from the pretraining stage, as the parameter representation changes; however, this does not impact training time significantly, because the pretraining stage is short.

%To generate these candidates, we must first automatically group layers where parameter sharing is most effective together.  Our approach is guided by the hypothesis that if two layers learn similar weights over the same set of candidates, so that the generated weights used by each layer end up being similar, then we can share weights between them with little (or no) performance degradation. 
%
%We begin by grouping together all layers so they all share the same parameters $\psi_i$.   
%
%To ensure each layer operates on the same set of candidates, we split $\psi_i$ into equal sized candidates $C$ (we found $|C|=4$ worked well).  Each candidate is reshaped to the size of $\theta_j$ for each layer, and then we learn a weighted combination using the generation methods in Section~\ref{subsec:generation}.
%
%After a few epochs, we perform K-means clustering on all the layer representations (\eg, the weights used to combine the candidates) and use the clusters to map layers to elements of $\Psi$ for training. 

%
%Each element is allocated a proportional number of parameters that is equivalent to its portion of the weights the group's layers represent. 
%
%For example, if a $\psi_i$ has two layers that each require 10K weights (20K total), and the total number of weights required by the entire network is 100K, then it would receive 20\% of the parameters allocated in the SSN.  After this pretraining step is complete, we train our SSN on the target task from scratch.

==> 7_broader_impact.tex <==
\section*{Broader Impact}

Shapeshifter Networks are a broad and general-purpose tool applicable to many downstream tasks. It is thus hard to identify specific impacts, as they are closely tied to the nature of the application Shapeshifter Networks are applied to. We instead will focus broadly on the impact of reducing the memory requirements for training and deploying models.

Given the current trend toward training ever-larger models, a technique that can capture the benefits of large models without their memory requirements has many potentially positive impacts. As data movement is now the dominant factor in both energy consumption and performance~\cite{unat2017trends}, reducing it can help improve the efficiency and reduce the energy costs of models both during training and deployment. This would be a positive step toward reducing the environmental impact of machine learning~\cite{strubell2019energy,schwartz2019green}. Further, being able to train models without requiring the resources of a large cluster helps to democratize deep learning and make it more accessible to communities.

However, these same benefits can be a double-edged sword, allowing potentially-harmful applications to be cheaply and widely deployed (\eg, surveillance). While this is a risk shared with any technique that improves the efficiency of deep learning, we feel it is important to acknowledge it. We would specifically encourage future research on the impact of increasingly powerful yet increasingly efficient machine learning systems, especially in combination with the improved efficiency of dedicated acceleration hardware.

==> saved.tex <==

As discussed in the Introduction, we can obtain a more efficient parameter representation by learning to combine a set of basis filters to create the filter patterns required by layers in a network (see Figure~\ref{fig:filters} for an example).  Prior work used a set of hand-crafted heuristics that learned this decomposition for identical layers in a network~\cite{bai2019deep,dehghani2018universal,Lan2020ALBERT,savarese2018learning}, which makes them ill-suited for Learning APART, as discussed in Section~\ref{subsec:challenges}.  In contrast, our Shapeshifter Networks (SSNs), automatically learns to where and how to share parameters in a network.  Essentially, our SSNs can take any number of parameters and morph them to fit the weights desired by a network architecture.  There are two problems that we have to address to accomplish this feat effectively, which have not been investigated in prior work.  First, we learn how to automatically identify the layers where parameter sharing is effective (Section~\ref{subsec:selector}). Second, we learn to generate weights, even when layers request more parameters than are available (Section~\ref{subsec:upsample}).

%We now describe Shapeshifter Networks in detail. 
%
%A simple feed-forward network like those in Figure~\ref{fig:parameter_sharing} can be thought of as applying $L$ layer operations $f_{\{1,...,L\}}$ to input data $x$ given model parameters $\theta$. For simplicity, we present this case and also neglect layers that do not require parameters, but our approach is applicable to any architecture.  
%\htor{this sounds limiting, it would also work for recurrent or skip conns, no?}
%
%For simplicity, we ignore layers that do not require model parameters like activation functions. 
%
%A traditional neural network would implicitly choose the layer parameters for each learnable operation $f_i$.
%
%In contrast, SSNs decouple the $f_i$ from their parameters, and instead query a parameter store (Section~\ref{subsec:allocator}) to obtain weights to perform its operation.  Parameters from regularization layers such as Batch Normalization~\cite{IoffeBatchNorm2015} are not shared with other layers.  We note these layers typically have a negligible contribution to the number of parameters in a neural network, but all other operations requiring parameters may end up sharing weights.  Some layers may require a parameter store to perform weight upsampling (Section~\ref{subsec:upsample}) when it needs more weights than are available. In addition, some layers may find sharing parameters detrimental to performance, and so we learn to split layers into parameter groups (Section~\ref{subsec:groups}).  Each group has its own parameter store (\ie, parameters are not shared between groups).   SSNs do not require modifying a network's architecture or its loss function, making them easy to adapt to any task or network.
%
%SSNs make no prior assumptions about a model's architecture, so they can be used to implement any neural network with arbitrary numbers of parameters.


%A traditional neural network could be implemented using our framework by placing each layer in its own parameter group and then allocate the minimum number of parameters required to implement each operation.  However, a Shapeshifter network need not be contrained in such a manner, layers may

\subsection{Selecting Parameters from a Parameter Store}
\label{subsec:selector}

In a SSN all trainable parameters are managed by a parameter store.  Given a network architecture, the parameter store's job is to select the parameters that are used by each layer to generate its weights.  More formally, a parameter store has a set of trainable parameters $\psi_i \in \Psi$ used to generate weights for layers.  Each element $\psi_i$ represents a vector of parameters, and any layers that are associated with the same $\psi_i$ may share parameters. Let $D_1^j, \ldots, D_M^j$ be the dimensions of the parameters $\theta_j$ needed by a network architecture's $j$th layer. We obtain a candidate set of $P$ templates for layer $j$, $C_j \in \mathbb{R}^{P, D_1^j, ..., D_M^j}$, by reshaping its $\psi_i$ (ignoring excess).  If too few parameters are available for a single candidate, we use parameter upsampling (Section~\ref{subsec:upsample}).  Note that we may provide $P$ as a hyperparameter, which may be smaller than the number of candidates that can be constructed from $\psi_i$.  In this case, we allocate candidates in a round robin fashion to construct $C_j$.  Once we have selected the candidates for a layer, we learn a weighted combination of them to generate its weights (described in Section~\ref{subsec:upsample}).

To generate these candidates, we must first automatically group layers where parameter sharing is most effective together.  Our approach is guided by the hypothesis that if two layers learn similar weights over the same set of candidates, so that the generated weights used by each layer end up being similar, then we can share weights between them with little (or no) performance degradation. 
%
We begin by grouping together all layers so they all share the same parameters $\psi_i$.   
%
To ensure each layer operates on the same set of candidates, we split $\psi_i$ into equal sized candidates $C$ (we found $|C|=4$ worked well).  Each candidate is reshaped to the size of $\theta_j$ for each layer, and then we combine them using the generation methods in Section~\ref{subsubsec:learned_allocation}.
%
After a few epochs, we perform K-means clustering on all the layer representations (\eg, the weights used to combine the candidates) and use the clusters to map layers to elements of $\Psi$ for training. 

%
Each element is allocated a proportional number of parameters that is equivalent to its portion of the weights the group's layers represent. 
%
For example, if a $\psi_i$ has two layers that each require 10K weights (20K total), and the total number of weights required by the entire network is 100K, then it would receive 20\% of the parameters allocated in the SSN.  After this pretraining step is complete, we train our SSN on the target task from scratch.
%
%As our experiments will show, this typically performs at least on par, and often better than manually created groups, while being applicable to \emph{any} network and also providing much greater flexibility number and makeup of the groups that are produced.

%Traditional parameter sharing assumes each layer has identical dimensions and performs the same operation.  While a naive parameter sharing strategy effectively sets $P=1$, Savarese~\etal~\cite{savarese2018learning} showed that learning a weighted combination of candidates $C_j$ could improve performance, although they also only considered a setting where layers were the same size/type. We benchmark their approach and three other strategies for combining these candidates when $P > 1$ in our more general setting where parameter sharing can occur between any layer.  We categorize these into simple methods that extract parameters directly from $C_j$ (Section~\ref{subsubsec:direct_allocation}) and methods that learn a unique combination of the candidates $C_j$ for each layer to obtain $\theta_j$ (Section~\ref{subsubsec:learned_allocation}).

%\begin{figure*}
%    \centering
    % Editing link to figure: https://docs.google.com/drawings/d/1UKdzvDC6dqHG1SqFCXpRIfDiOqpajAgMe5oe5fNRcXk/edit?usp=sharing
    % TODO: make more compact, update notation 
    % \includesvg[width=\textwidth]{"figures/allocation_method_figure.svg"}
%    \includegraphics[width=0.9\textwidth]{"figures/combination_strategies.pdf"}
%    \caption{Illustration of the parameter selector (described in Section~\ref{subsec:allocator}) and candidate combination strategies (described in Section~\ref{subsubsec:direct_allocation} and Section~\ref{subsubsec:learned_allocation}).}
 %   \label{fig:allocation}
%\end{figure*}

\subsubsection{Direct Candidate Combination}
\label{subsubsec:direct_allocation}
Here we describe the strategies we employ that require no parameters to be learned by the parameter combiner, \ie, they operate directly on the candidates $C_j$.% The only hyperparameter that influences the selection is $P$, the maximum size of the candidate set $C$.
%\smallskip

\noindent\textbf{Round Robin (RR)} reuses parameters of each candidate set as few times as possible. The scheme simply returns the weights at index $i$ mod $|C_j|$ in the (ordered) candidate set $C_j$ at the $i$th query of a parameter store.
%\smallskip

\noindent\textbf{Candidate averaging (Avg)} averages all candidates in $C_j$ to provide a naive baseline for using multiple candidates. A significant drawback of this approach is that, if $|C_j|$ is large, this can result in reusing parameters (across combiners) many times with no way to adapt to a specific layer, especially when the size of the parameter group is small.  


\subsubsection{Learned Candidate Combination}
\label{subsubsec:learned_allocation}

We now describe strategies that use learned coefficients $\alpha_j$ to combine the candidates in set $C_j$.
%
Essentially, the goal is to use a soft-attention mechanism~\cite{bahdanau2015neural} over $C$ to obtain the layer parameters. %\htor{should we stop calling $C$ a set but rather a (stacked) tensor?}
%\ndryden{I think it is fine to logically describe it as a set.}
%
Each strategy begins with features $\phi_i$ representing each layer $i$. These features use an orthogonal initialization so that they begin as far from other layers' features as possible. Unlike the methods from Section~\ref{subsubsec:direct_allocation}, these allocation strategies use a few model parameters to combine candidates (typically less than $0.1\%$ of the total number of parameters in our experiments).
%\smallskip

\noindent\textbf{Candidate weighted averaging (WAvg)} uses a weighted average over available candidates, and was introduced by Savarese~\etal~\cite{savarese2018learning}.  The coefficients used to combine the candidates are directly learned for each layer. % and are forced to sum to 1, \ie, $\alpha_{j} = \mathrm{softmax}(\phi_{i})$. 
Then, the model weights are computed via:
\begin{equation}
    \theta_j = \sum_{k=1}^{|C_j|} \alpha_{jk} C_{jk}
    \label{eq:weight_sum}
\end{equation}
where $\theta_j$ is the weighted sum of each candidate.
%\smallskip

\noindent\textbf{Layer embeddings (Emb)} represent each layer by an embedding $\phi_i$ resulting in a $L \times |C_j| \times 24$ feature tensor.  From these embeddings we predict the coefficients $\alpha$ for combing the candidates using Eq.~(\ref{eq:weight_sum}) using a fully connected (FC) layer. Layers that operate over the same set of candidates use the same FC layer, which enables us to identify when layers can be implemented using similar parameters as their embeddings will end up near each other.  We did try to use a MLP with more layers and nonlinear activation functions, but it did not improve performance.  More formally, let $W_p$ and $b_p$ be the weights and bias of a FC layer with output dimension $|C_j|$. Then we obtain coefficients with:
\begin{equation}
    \alpha_j = \mathrm{softmax}(\phi_iW_p + b_p).
    \label{eq:emb_attention}
\end{equation}
%\htor{unclear, maybe specify exact tensor contraction that implements the embedding (at least in supp)?}

\subsection{Upsampling Weights in a Parameter Store}
\label{subsec:upsample}

One of the new challenges addressed in this work is how to effectively upsample the weights when a layer requests more parameters than are available in a store.  A naive approach would be simply to \textbf{repeat} parameters.  For example, if a FC layer asks for a $100 \times 100$ weight matrix, but the largest weight matrix the store can make is $50 \times 100$, one could simply make a copy and concatenate them together.  Another alternative would be to use \textbf{bilinear interpolation (inter)}.  However, both approaches are clearly not satisfying, as they would create redundancies or limit the kinds of patterns the parameters could capture in the data.  As such, %in addition to these two naive baselines, 
we introduce a method that learns how to modify the parameters in order to capture new concepts.
%For each method, we first use all the parameters available in a store.  When additional parameters are needed we either upsample the parameters using Inter, or we concatenate the unmodified parameters together additional parameters generated with Repeat or from our parameters below. These modifications are built over parameter windows, \ie, a set of weights in sequence in a store.  By default we group together parameters in sets of 9 (for a 3x3 kernels which if often used in many layers in modern CNNs), which we found to work well.  We refer to these parameter sets as filters for ease of notation. 
%\smallskip

%\noindent\textbf{Weighted combination.}  We extend our weighted combination strategy (Eq.~(\ref{eq:weight_sum})) to create new parameters by combining multiple filters.  This approach requires very few additional parameters, since it simply requires us to learn a single weight for each filter.
%\noindent\textbf{Learned linear modification (Linear).}  We use a fully connected layer that takes one or more filters as input and outputs a new set of filters.  For example, we can use a fully connected layer to take a single filter as input and output a new filter (\ie, it has an input and output dimension of 9).  We also explored using ReLU activations as well, but it did not improve performance.  However, this kind of approach can be computationally expensive and even relatively small modifications could require quite a few parameters (\eg, if we took 20 filters as input to create 20 new filters it would require $180 \times 180 = 32,400$ parameters).  While this may be negligible for very large networks with many parameters, if our goal is to create a compact network with only a few hundred thousand parameters this could be very expensive, while also potentially being in high demand.
%\smallskip

\noindent\textbf{Masking filters (Mask).} With this method, we first use all available parameters in a store for the candidate, and then upsample by concatenating windows of parameters (\ie, sets of sequential parameters) multiplied element-wise by a learned mask. By default, we group parameters in windows of size 9 (for the commonly-used $3 \times 3$ kernels in CNNs), which we found to work well, but any size can be used. Note that even if several masks are required to learn multiple alterations of parameters, only a negligible number of learned parameters are required.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{figures/models.pdf}
    \caption{Examples of architectures used to evaluate SSNs. Fully connected (FC) and bidirectional GRU (Bi-GRU) layers give their $in \times out$ dimensions; convolutional layers (conv) give the number of layers, kernel size, and number of filters.  Same colored boxes show ``manual'' (Table~\ref{tab:groups}) sharing, except for green boxes in WRN, whose layers share no parameters. Layers without parameters omitted.}
    \label{fig:models}
\end{figure*}

\subsection{Learning Parameter Groups}
\label{subsec:groups}

Determining where parameter sharing is beneficial is a precondition in any parameter sharing scheme.  We refer to layers that share parameters as \emph{parameter groups}, each of which has its own parameter store (so they do not share parameters with layers from other groups).
%Some layers in a neural network may inherently perform very similar operations, which enables parameter sharing with little performance loss.
%
%However, the inputs to some layers may vary drastically, requiring very different model parameters, which can lead to performance degradation if the same parameters are used to represent all of them.
%For example, early layers, which are typically associated with learning low-level features, may hurt performance if shared with late layers that are often associated with higher-level concepts.
%
Prior work uses architecture or task specific heuristics that all stipulate that only identical layers can form a group (\eg,~\cite{bai2019deep,Lan2020ALBERT,savarese2018learning}). Thus, prior work has little or no benefit for architectures with few (or no) identical layers.  For example, DenseNet~\cite{Huang_2017_CVPR} concatenates the activations of prior layers into new layers (\ie, each layer is inherently larger than the previous ones).  Many neural networks that use multiple modalities (\eg, vision-language tasks) also often have few layers of the same size/type, and parameter sharing may be difficult even when there are identical layers.  For example, the identical (FC) layers in ADAPT-T2I~\cite{Wehrmann_2020_AAAI} take the same language features as input, and then predict the shifting and scaling weights used to modify image features.  In other words, they have the same input, but require different outputs, making parameter sharing problematic. 
%
%However, this kind of approach is overly restrictive by requiring a specific number of parameter groups, and may significantly reduce performance if the groups it chooses have too few parameters for their layers, resulting in frequent weight upsampling.
%

We avoid the overly restrictive parameter sharing schemes in prior work by automatically learning where parameter sharing is most effective.
%
Our approach is guided by the hypothesis that if two layers learn a similar layer representation $\phi$ when they operate on the same set of candidates, so that the weights used by each layer end up being similar, then we can share weights between them with little (or no) performance degradation. 
%
We begin by grouping together all layers so they all share the same parameter store (\ie, they are in the same parameter group).   
%
To ensure each layer operates on the same set of candidates, we split the store's parameters into equal sized candidates $C$ (we found $|C|=4$ worked well).  Each candidate is reshaped to the size of $\theta_j$ for each layer, and then we combine them using Eq.~(\ref{eq:weight_sum}) using either the Emb or WAvg strategies from Section~\ref{subsubsec:learned_allocation}.
%
After a few epochs, we perform K-means clustering on all the layer representations $\phi$ (\emph{not} the weights $\theta$) and use the clusters as a our parameter groups for training. 

%
Each group is allocated a proportional number of parameters that is equivalent to its portion of the weights the group's layers represent. 
%
For example, if a parameter group has two layers that each require 10K weights (20K total), and the total number of weights required by the entire network is 100K, then it would receive 20\% of the parameters allocated in the SSN.  After we create our parameter groups and allot weights to groups, we train our SSN on our target task from scratch.
%
As our experiments will show, this typically performs at least on par, and often better than manually created groups, while being applicable to \emph{any} network and also providing much greater flexibility number and makeup of the groups that are produced.

==> saved_experiments.tex <==

\section{Experiments}

We provide experiments across a wide variety of tasks and networks in order to demonstrate the broad applicability of our SSNs.
%
%Section~\ref{subsec:tasks} provides a brief overview of the tasks and methods that we train using our new framework which we discuss in Section~\ref{subsec:results}.  Finally, we further illustrate the benefits of our approach on the knowledge distillation task in Section~\ref{subsec:distillation}.
%
We adapt code and data splits made available by the authors and report the average of five runs for all comparisons except ImageNet, which averages three runs.

\begin{figure*}
    \centering
    %\includegraphics[width=0.3\textwidth]{figures/bidir_ret.pdf}\hspace{3mm}
    \includegraphics[width=0.48\textwidth]{figures/cifar100.pdf}\hspace{3mm}
    \includegraphics[width=0.48\textwidth]{figures/imagenet.pdf}
    \caption{Comparison of reducing the parameter parameters by adjusting layer sizes vs.\ our SSNs using the same number of parameters.  We also compare to SWRN~\cite{savarese2018learning}, prior work leveraging parameter sharing that is unable to use fewer than 33\% of the parameters of a fully-parameterized WRN-28-10.  In contrast, we can not only use far fewer parameters that perform better than SWRN, but we can also implement even larger networks (WRN-76-12) without having to increase our parameter usage. See text for additional discussion.}
    \label{fig:param_reduce_compare}
    \vspace{-0.5em}
\end{figure*}



\subsection{Compared Tasks}
\label{subsec:tasks}
Below we briefly describe each task, datasets, and evaluation metrics.  For each model, we use the author's implementation, following their hyperparameter settings, except where noted (additional details in the supplementary).% Our baseline versions match or exceed prior results for these networks/datasets.

\noindent\textbf{Image Classification.}
For image classification the goal is to recognize if an object is present in an image. This is evaluated using Error@$k$, \ie, the portion of times that the correct category does not appear in the top $k$ most likely objects.  We evaluate SSNs on CIFAR-10 and CIFAR100~\cite{cifar}, which are composed of 60K images of 10 and 100 categories, respectively, and ImageNet~\cite{deng2009imagenet}, which is composed of 1.2M images containing 1,000 categories.  We report Error@1 on CIFAR and Error@5 for ImageNet. 
\smallskip

\noindent\textbf{Image-Sentence Retrieval.}
Given an image the goal in image-sentence retrieval is to retrieve a relevant sentence and vice versa.  This task is evaluated using Recall@K=\{1, 5, 10\} for both directions (six numbers), which we average for simplicity.  We compare methods on two datasets: Flickr30K~\cite{young2014image} which contains 30K/1K/1K images for training/testing/validation, each with five descriptive captions, and COCO~\cite{lin2014microsoft}, which contains 123K/1K/1K images for training/testing/validation, each image with about five descriptive captions. We evaluate SSNs using EmbNet~\cite{Wang_2016_CVPR} and ADAPT-T2I~\cite{Wehrmann_2020_AAAI} (Figure~\ref{fig:models}(a,c)).  Note that, as discussed in Section~\ref{subsec:groups} ADAPT-T2I has identical parallel layers (layers that need different outputs despite having the same input), which makes sharing parameters challenging.
\smallskip

%\noindent\textbf{EmbNet~\cite{Wang_2016_CVPR}.}   This network learns to embed visual features for each image computed using a 152-layer Deep Residual Network (ResNet)~\cite{he2016deep} that has been trained on ImageNet~\cite{deng2009imagenet} and MT GrOVLE~\cite{burnsLanguage2019} language features into a shared semantic space using a triplet loss.  The network consists of two branches, one for each modality, and each branch contains two fully connected layers (for a total of four layers).

%\noindent\textbf{ADAPT-T2I~\cite{Wehrmann_2020_AAAI}.} In this approach word embeddings are aggregated using a bidirectional GRU~\cite{cho-etal-2014-learning} and its hidden state at each timestep is averaged to obtain a full-sentence representation.  Images are represented using 36 bottom-up image region features~\cite{Anderson_2018_CVPR} that are passed through a fully connected layer.  Then, each sentence calculates scaling and shifting parameters for the image regions using a pair of fully connected layers that both take the full-sentence representation as input.  The image regions are then averaged, and a similarity score is computed between the sentence-adapted image features and the fully sentence representation.  Thus, there are four layers total (3 fully connected, 1 GRU) that can share parameters, including the two parallel fully connected layers (\ie, they both take the full sentence features as input, but are expected to have different outputs).

\midsepremove{}
\begin{table}%[htb!]
  \centering
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{ll|ccc}
    \toprule
    Dataset  & Method & \multicolumn{3}{c}{Performance} \\
    \midrule
    \multicolumn{2}{l|}{\textbf{Image-Sentence Retrieval}} & & & \\
    \cmidrule{1-5}
    \multicolumn{2}{r|}{\% orig params} & 6.9\% & 13.9\% & 100\% \\
    \cmidrule{1-5}
    \multirow{2}{*}{F30K~\cite{young2014image}} & EmbNet~\cite{Wang_2016_CVPR} & 56.5 & 70.2 & 74.1 \\
             & SSN-EmbNet & \textbf{67.9} & \textbf{71.6} & \textbf{74.4} \\
    \cmidrule{1-5}
    \multirow{2}{*}{COCO~\cite{lin2014microsoft}} & EmbNet~\cite{Wang_2016_CVPR} & 74.2 & 77.3 & 81.4 \\
             & SSN-EmbNet & \textbf{76.7} & \textbf{78.2} & \textbf{82.1} \\
    \cmidrule{1-5}
    \multicolumn{2}{r|}{\% orig params} & 34.7\% & 70.9\% & 100\% \\
    \cmidrule{1-5}
    \multirow{2}{*}{F30K~\cite{young2014image}} & ADAPT-T2I~\cite{Wehrmann_2020_AAAI} & 76.6 & 80.6 & \textbf{83.3} \\
             & SSN-ADAPT-T2I & \textbf{81.2} & \textbf{81.7} & 82.9 \\
    \cmidrule{1-5}
    \multirow{2}{*}{COCO~\cite{lin2014microsoft}} & ADAPT-T2I~\cite{Wehrmann_2020_AAAI} & 83.8 & 85.2 & 86.8 \\
             & SSN-ADAPT-T2I & \textbf{85.3} & \textbf{86.2} & \textbf{87.0} \\
    \midrule
    \multicolumn{2}{l|}{\textbf{Phrase Grounding}} & & & \\
    \cmidrule{1-5}
    \multicolumn{2}{r|}{\% orig params} & 7.8\% & 15.6\% & 100\% \\
    \cmidrule{1-5}
    \multicolumn{1}{c}{F30K} & SimNet~\cite{wang2018learning} & 70.6 & 71.0 & 71.7 \\
    Entities~\cite{flickrentitiesijcv} & SSN-SimNet & \textbf{71.9} & \textbf{72.1} & \textbf{72.4} \\
    \cmidrule{1-5}
    \multirow{2}{*}{ReferIt~\cite{kazemzadeh-EtAl:2014:EMNLP2014}} & SimNet & 58.5 & 59.2 & \textbf{61.1} \\
             & SSN-SimNet & \textbf{59.5} & \textbf{59.9} & 61.0 \\
    \bottomrule
  \end{tabular}
  \caption{Performance of SSNs vs.\ traditional networks of a comparable size on image-sentence retrieval and phrase grounding.}
  \label{tab:vl_models}
\end{table}
\midsepdefault{}

\midsepremove{}
\begin{table}[t]%[htb!]
  \centering
  \setlength{\tabcolsep}{2pt}
  \begin{tabular}{l|c|c|c}
    \toprule
    \multirow{2}{*}{Method} & CIFAR-10~\cite{cifar} & \% original & \% original \\
                            & Error@1 & test FLOPs & test params \\
    \midrule
    ResNet-56~\cite{he2016deep} & 6.74 & 100 & 100\\
    L1~\cite{li2017pruning} & 6.94 & 72.4 & 85.9\\
    HRank~\cite{Lin_2020_CVPR} & 6.48 & 70.7 & 83.2\\
    NISP~\cite{Yu_2018_CVPR} & 6.99 & 64.5 & 57.6\\
    C.\ Prune~\cite{He_2017_ICCV} & 9.20 & 50.6 & --\\
    HRank~\cite{Lin_2020_CVPR} & 10.75 & \textbf{20.3} & 28.4\\
    \midrule
    SSN- & 9.26 & 100 & \textbf{12.2}\\
    SSN+ & \textbf{5.21} & 100 & 100\\
    HRank \& SSN+ & 5.86 & 70.7 & 83.2\\
    HRank \& SSN+ & 9.94 & \textbf{20.3} & 28.4\\
    \bottomrule
  \end{tabular}
  \caption{Comparison of SSNs to parameter pruning methods. We use either relatively few parameters (SSN-), or we use additional parameters during training and then precompute each layer's weights at test time to remove any overhead (SSN+).  Note that parameter pruning methods only reduce test time computational resources, and do not save GPU memory during training like SSNs.}
  \label{tab:pruning}
\end{table}
\midsepdefault{}


\noindent\textbf{Phrase Grounding.}
In phrase grounding the goal is to find the image region described by a given phrase.  Performance is measured by how often the predicted box for a phrase has at least 0.5 intersection over union with its ground truth box.  We evaluate on Flickr30K Entities~\cite{flickrentitiesijcv} which augments Flickr30K with 276K bounding boxes for phrases in image captions, and ReferIt~\cite{kazemzadeh-EtAl:2014:EMNLP2014}, which contains 20K images that are evenly split between training/testing and 120K region descriptions.  We evaluate our SSNs with SimNet~\cite{wang2018learning} (Figure~\ref{fig:models}(b)) using the implementation from Plummer~\etal~\cite{plummerPhraseDetection} that reports state-of-the-art results on this task.


%\noindent\textbf{SimNet~\cite{wang2018learning}.}  This network contains three branches that each operate on different types of features.  One branch passes image regions features computed with a 101-layer ResNet that have been fine-tuned for phrase grounding~\cite{plummerPhraseDetection} using two fully connected layers.  A second branch passes MT GrOVLE features through two fully connected layers.  Then, a joint representation is computed for all region-phrase pairs using an elementwise product.  Finally, the third branch passes these joint features through three fully connected layers (7 total), where the final layer acts as a classifier indicating the likelihood that phrase is present in the image region.

\midsepremove{}
\begin{table*}
    \centering
    \begin{tabular}{c|cc|cc|c}
    \toprule
    Experiment & Teacher & \#Params (M) & Student  & \#Params (M) & Dataset\\
    \midrule
        (a) & WRN-28-4 & 5.87 & WRN-28-2 & 1.47 & CIFAR-100\\
        (b) & WRN-28-4 & 5.87 & WRN-16-2 & 0.70 & CIFAR-100\\
    \bottomrule
    \end{tabular}
    \caption{Experimental setup for our knowledge distillation experiments reported in Table~\ref{tab:distill_groups}.}
    \label{tab:distill_setup}
\end{table*}
\midsepdefault{}

\midsepremove{}
\begin{table*}[htb!]
    \centering
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{c|c|c|ccccc|cc}
    \toprule
    Experiment & Teacher & Baseline & AT~\cite{Zagoruyko2017AT} & Jacobian~\cite{SrinivasJacobianICML2018} & FT~\cite{kimFactorTransfer2018} & AB~\cite{ABdistill} & OD~\cite{Heo_2019_ICCV} & SSN+ (ours) & OD \& SSN+\\
    \midrule
        (a) & 21.09 & 24.88 & 23.80 & 23.70 & 23.41 & 23.19 & 21.98 & 23.62 & \textbf{21.21}\\
        (b) & 21.09 & 27.32 & 26.56 & 26.71 & 25.91 & 26.02 & 24.08 & 26.53 & \textbf{23.30}\\
    \bottomrule
    \end{tabular}
    \caption{Knowledge distillation results on CIFAR-100 using setup in Table~\ref{tab:distill_setup}.  Note SSNs only use a teacher when combined with OD~\cite{Heo_2019_ICCV}.}
    \label{tab:distill_groups}
\end{table*}
\midsepdefault{}

\midsepremove{}
\begin{table*}[htb!]
  \centering
  \setlength{\tabcolsep}{2pt}
  \begin{tabular}{l|ccl|c|cccc}
    \toprule
    & Orig Num & \% of Params &  & Reduced &  \multicolumn{4}{c}{SSN Variants (ours)} \\
    \cmidrule{6-9}
    Method & Params (M) & Used & Dataset & Baseline & RR & Avg & WAvg & Emb\\
    \midrule
    \multicolumn{3}{l}{\textbf{Image-Sentence Retrieval}} & & \multicolumn{5}{c}{(higher numbers are better)} \\
    \cmidrule{1-9}
    % & \#Params (M) & 7 & 4& 4 & 4 & 4 & 4 \\
    \multirow{2}{*}{EmbNet~\cite{Wang_2016_CVPR}} & \multirow{2}{*}{7} & \multirow{2}{*}{57.1\%} & F30K~\cite{young2014image} & 72.8 & 74.1 & 73.5 & 74.0 & \textbf{74.3} \\
    & & & COCO~\cite{lin2014microsoft} & 80.9 & 80.8 & 80.9 & 81.2 & \textbf{81.5} \\
    \cmidrule{1-9}
    % & \#Params (M) & 14 & 10 & 10 & 10 & 10 & 10 \\
    \multirow{2}{*}{ADAPT-T2I~\cite{Wehrmann_2020_AAAI}} & \multirow{2}{*}{14} & \multirow{2}{*}{70.9\%} & F30K~\cite{young2014image} & 80.6 & 81.2 & 80.5 & 81.6 & \textbf{81.7} \\
    & & &  COCO~\cite{lin2014microsoft} & 85.2 & 85.6 & 85.8 & \textbf{86.2} & 85.9 \\
    \midrule
    \multicolumn{3}{l}{\textbf{Phrase Grounding}} & & \multicolumn{5}{c}{(higher numbers are better)} \\
    \cmidrule{1-9}
    % &\#Params (M) & 6 & 2 & 2 & 2 & 2 & 2\\
    \multirow{2}{*}{SimNet~\cite{wang2018learning}} & \multirow{2}{*}{6} & \multirow{2}{*}{33.1\%} & F30K Entities~\cite{flickrentitiesijcv} & 71.1 & 72.3 & 72.1 & 72.3 & \textbf{72.5} \\
    & & & ReferIt~\cite{kazemzadeh-EtAl:2014:EMNLP2014} & 59.4 & \textbf{60.5} & 60.2 & \textbf{60.5} & 60.4\\
    \midrule
    \multicolumn{3}{l}{\textbf{Image Classification}} & & \multicolumn{5}{c}{(lower numbers are better)}\\
    \cmidrule{1-9}
    % & \#Params (M) & 36/69 & 4/19 & 4/19 & 4/19 & 4/19 & 4/19\\
    \multirow{2}{*}{WRN-28-10~\cite{Zagoruyko2016WRN}} & \multirow{2}{*}{36} & \multirow{2}{*}{11.3\%} & CIFAR-10~\cite{cifar} & 4.22 & 4.09 & 4.19 & 4.00 & \textbf{3.84} \\
    & & & CIFAR-100~\cite{cifar} & 22.34 & 21.91 & 22.78 & \textbf{21.78} & 21.92 \\
    \cmidrule{1-9}
    WRN-50-2~\cite{Zagoruyko2016WRN} & 69 & 27.5\% & ImageNet~\cite{deng2009imagenet} & 10.08 & \textbf{6.69} & 7.61 & 7.38 & \textbf{6.69} \\
    \bottomrule
  \end{tabular}
  \caption{Parameter combination method comparison (see Section~\ref{subsec:allocator} descriptions).  All models in the same row use the same (reduced) number of parameters.  ``Reduced Baseline'' uses no parameter sharing, but adjusts the number and/or size of filters so they have the same number of parameters as our SSNs.  The original model's performance is reported in the first column of results in Table~\ref{tab:groups}.}
  \label{tab:allocation}
\end{table*}
\midsepdefault{}

\midsepremove{}
\begin{table*}[t]
  \centering
  \setlength{\tabcolsep}{2pt}
  \begin{tabular}{l|cl|c|ccccc}
    \toprule
    &  &  &  & \multicolumn{5}{c}{SSN Variants (ours)} \\
    \cmidrule{5-9}
    Method & \#Groups & Dataset & Baseline & Single & Random & Manual & WAvg & Emb \\
    \midrule
    \multicolumn{3}{l|}{\textbf{Image-Sentence Retrieval}} & \multicolumn{6}{c}{(higher numbers are better)} \\
    \cmidrule{1-9}
    \multirow{2}{*}{EmbNet~\cite{Wang_2016_CVPR}} & \multirow{2}{*}{2} & F30K~\cite{young2014image} & 74.1 & \textbf{74.4} & 74.0 & 74.3 & 74.2 & 74.3 \\
    & & COCO~\cite{lin2014microsoft} & 81.4 & \textbf{82.1} & 81.5 & 81.7 & 81.7 & 81.9 \\
    \cmidrule{1-9}
    \multirow{2}{*}{ADAPT-T2I~\cite{Wehrmann_2020_AAAI}} & \multirow{2}{*}{2} & F30K~\cite{young2014image} & \textbf{83.3} & 82.1 & 81.9 & 82.0 & 82.6 & 82.9 \\
    & & COCO~\cite{lin2014microsoft} & 86.8 & 86.1 & 86.3 & 86.1 & 86.4 & \textbf{87.0} \\
    \midrule
    \multicolumn{3}{l|}{\textbf{Phrase Grounding}} & \multicolumn{6}{c}{(higher numbers are better)} \\
    \cmidrule{1-9}
    \multirow{2}{*}{SimNet~\cite{wang2018learning}} & \multirow{2}{*}{3} & F30K Entities~\cite{flickrentitiesijcv} & 71.7 & 71.4 & 71.8 & \textbf{72.4} & 72.2 & 72.1 \\
    & & ReferIt~\cite{kazemzadeh-EtAl:2014:EMNLP2014} & \textbf{61.1} & 60.9 & 60.0 & 60.2 & 61.0 & 60.5 \\
    \midrule
    \multicolumn{3}{l|}{\textbf{Image Classification}} & \multicolumn{6}{c}{(lower numbers are better)} \\
    \cmidrule{1-9}
    \multirow{2}{*}{WRN-28-10~\cite{Zagoruyko2016WRN}} & \multirow{2}{*}{14} & CIFAR-10~\cite{cifar} & 3.57 & 3.71 & 3.63 & \textbf{3.38} & 3.51 & 3.42 \\
    & & CIFAR-100~\cite{cifar} & 19.44 & 19.99 & 20.36 & 19.29 & 19.47 & \textbf{19.24} \\
    \cmidrule{1-9}
    WRN-50-2~\cite{Zagoruyko2016WRN} & 32 & ImageNet~\cite{deng2009imagenet} & 5.84 & 6.18 & 5.91 & \textbf{5.82} & 5.86 & 5.96 \\
    \bottomrule
    % \multirow{3}{*}{DenseNet~\cite{Huang_2017_CVPR}} & \multirow{3}{*}{100/} & CIFAR-10+~\cite{cifar} & 2.98\\
    % & & CIFAR-100+~\cite{cifar} & 17.46\\
    % & & ImageNet~\cite{deng2009imagenet} & \\
    % \hline
  \end{tabular}
  \caption{Parameter bank grouping comparison (methods described in Section~\ref{subsec:groups}).  Each method uses the same number of parameters and the baseline represents no parameter sharing.  Notably, these results demonstrate how our automatically learned groups can provide greater flexibility when sharing parameters while performing on par or better than manually created groups (which are illustrated in Figure~\ref{fig:models}).}
  \label{tab:groups}
\end{table*}
\midsepdefault{}

\midsepremove{}
\begin{table*}[t]
  \centering
  \setlength{\tabcolsep}{2pt}
  \begin{tabular}{l|ccl|c|cccc}
    \toprule
    & Orig Num & \% of Params &  & Reduced & \multicolumn{4}{c}{SSN Variants (ours)} \\
    \cmidrule{6-9}
    Method & Params (M) & Used & Dataset & Baseline & Repeat & Inter  & Mask & 2 Groups+Mask \\
    \midrule
    \multicolumn{3}{l}{\textbf{Image-Sentence Retrieval}} & & \multicolumn{5}{c}{(higher numbers are better)} \\
    \cmidrule{1-9}
    % & \#Params (M) & 7 & 4& 4 & 4 & 4 & 4 \\
    \multirow{2}{*}{EmbNet~\cite{Wang_2016_CVPR}} & \multirow{2}{*}{6} & \multirow{2}{*}{6.9\%} & F30K~\cite{young2014image} & 56.5 & 64.8 & 67.5 & 67.3 & \textbf{67.9} \\
    & & & COCO~\cite{lin2014microsoft} & 74.2 & 75.5 & 76.1 & 76.2 & \textbf{76.7}\\
    \cmidrule{1-9}
    % & \#Params (M) & 14 & 10 & 10 & 10 & 10 & 10 \\
    \multirow{2}{*}{ADAPT-T2I~\cite{Wehrmann_2020_AAAI}} & \multirow{2}{*}{14} & \multirow{2}{*}{34.7\%} &  F30K~\cite{young2014image} & 76.6 & 79.0 & 80.9 & 80.3 & \textbf{81.2} \\
    & & &  COCO~\cite{lin2014microsoft} & 83.8 & 84.9 & \textbf{85.3} & 84.6 & 84.9 \\
    \midrule
    \multicolumn{3}{l}{\textbf{Phrase Grounding}} & & \multicolumn{5}{c}{(higher numbers are better)} \\
    \cmidrule{1-9}
    % &\#Params (M) & 6 & 2 & 2 & 2 & 2 & 2\\
    \multirow{2}{*}{SimNet~\cite{wang2018learning}} & \multirow{2}{*}{6} & \multirow{2}{*}{7.8\%} & F30K Entities~\cite{flickrentitiesijcv} & 70.6 & 71.1 & 71.8 & 71.5 & \textbf{71.9}\\
    & & & ReferIt~\cite{kazemzadeh-EtAl:2014:EMNLP2014} & 58.5 & 58.9 & 59.3 & 59.2 & \textbf{59.5}\\
    \midrule
    \multicolumn{3}{l}{\textbf{Image Classification}} & & \multicolumn{5}{c}{(lower numbers are better)} \\
    \cmidrule{1-9}
    % & \#Params (M) & 36/69 & 4/19 & 4/19 & 4/19 & 4/19 & 4/19\\
    \multirow{2}{*}{WRN-28-10~\cite{Zagoruyko2016WRN}} & \multirow{2}{*}{36} & \multirow{2}{*}{1.4\%} & CIFAR-10~\cite{cifar} & 6.35 & 5.43 & 6.05 & 5.18 & \textbf{5.07} \\
    & & & CIFAR-100~\cite{cifar} & 28.35 & 27.08 & 26.84 & 25.71 & \textbf{25.20} \\
    \cmidrule{1-9}
    WRN-50-2~\cite{Zagoruyko2016WRN} & 69 & 2.2\% & ImageNet~\cite{deng2009imagenet} & 15.20 & \textbf{14.16} & 14.83 & 14.19 & 14.58 \\
    \bottomrule
  \end{tabular}
  \caption{Parameter upsampling comparison (see Section~\ref{subsec:upsample} upsampling method descriptions). ``Reduced Baseline'' uses no parameter sharing, but adjusts the number and/or size of filters so they have the same number of parameters as our SSNs.  The original model's performance is reported in the first column of results in Table~\ref{tab:groups}.}
  \label{tab:upsample}
\end{table*}
\midsepdefault{}

%\noindent\textbf{Wide Residual Network (WRN)~\cite{Zagoruyko2016WRN}.}  WRN modified the traditional ResNets by increasing the width $k$ of each layer while also decreasing the depth $d$, which they found improved performance.  Different variants are  identified using WRN-$d$-$k$.  Following Savarese~\etal~\cite{savarese2018learning}, we evaluate our Shapeshifter Networks using WRN-28-10 for CIFAR and WRN-50-2 for ImageNet.

%\noindent\textbf{DenseNet~\cite{Huang_2017_CVPR}.} Unlike traditional neural networks where each layer in the network is computed in sequence, every layer in a DenseNet using feature maps from every layer which came before it.  Unlike WRN, these networks provide insight into the effect depth has on Shapeshifter networks, as we use a 190-layer DenseNet-BC configuration for CIFAR and a 161-layer DenseNet for ImageNet.


\subsection{Results}
\label{subsec:results}


In Figure~\ref{fig:param_reduce_compare}  we report results using our SSNs for image classification and Table~\ref{tab:vl_models} contains results on image-sentence retrieval and phrase grounding.  For each task and architecture we compare SSNs using the best settings from Section~\ref{subsec:ssn-analysis} (full details are in the supplementary) to a same sized network that does not share parameters.  Note the SWRN~\cite{savarese2018learning} sharing method cannot train a model with fewer than 12M parameters when implementing a Wide ResNet (WRN) 28-10~\cite{Zagoruyko2016WRN} (since it cannot share parameters between layers of different sizes/types).  However, in Figure~\ref{fig:param_reduce_compare}(a) we show that we can create a high performing SSN-WRN-28-10 even when using 0.5M parameters on CIFAR-100, and actually outperform the 12M variant of SWRN when using just 9M parameters.  Figure~\ref{fig:param_reduce_compare}(b) and Table~\ref{tab:vl_models} both demonstrate that these benefits generalize to ImageNet and the vision-language tasks, resp. Especially notable is SSNs on bidirectional retrieval, where we see up to an 11\% gain on F30K, using few parameters.  This demonstrates that SSNs can implement large networks with lower memory requirements than is possible with current methods by effectively sharing parameters.% which enables us to train larger, better-performing networks on comparable computational resources.

As mentioned in the Introduction, parameter pruning and knowledge distillation can help create more efficient models at test time, although they can not reduce memory requirements during training like SSNs.  As shown in Table~\ref{tab:pruning} and Table~\ref{tab:distill_groups}, our approach can be used to accomplish a similar goal as these tasks.  We report a 1.5\% gain over pruning methods even when using less than half the parameters as state-of-the-art methods, and can improve performance over training a traditional neural network directly.  That said, in both tasks there are benefits of using the prior work in terms of higher task accuracy in knowledge distillation or requiring fewer floating point operations in the case of pruning.  However, we also show in the last two lines of Table~\ref{tab:pruning} and the last column of Table~\ref{tab:distill_groups} that our approach can be combined with prior work to improve performance on both tasks.  To the best of our knowledge no prior work has shown to benefit both pruning and distillation.

%Methods that address the parameter pruning task can also be used to create models that have low memory requirements at test time (although not during training, like SSNs can). As shown in Table~\ref{tab:pruning}, our SSNs outperform recent parameter pruning methods even when training a model with less than half the parameters, but our approach does require more floating point operations (FLOPS) than parameter pruning. However, we would like to reiterate that our SSNs can reduce memory during training and at test time, whereas parameter pruning methods assume they are provided with a trained model, so they only can reduce memory at test time.  In addition, parameter pruning methods often require new methods for each layer type they wish to prune~\cite{Zhang2020OneShot}, whereas SSN can be used with any layer or architecture.  Finally, in the last line of Table~\ref{tab:pruning} we show that by using additional parameters during training to add capacity to a network, our SSNs can be combined with pruning methods to boost performance while maintaining the same test time memory and FLOP benefits as pruning alone.

%As mentioned in the Introduction, this idea of using additional computational resources during training to create a small high performing model is also similar to knowledge distillation.  In this task most methods take a high performing (teacher) network and transfer knowledge to a computationally efficient (student) network.  By comparison, when using extra model parameters our SSNs take a large model and directly learn to compress its weights to implement the small network.  As shown in Table~\ref{tab:pruning} and Table~\ref{tab:distill_groups} this can result in our SSN model performing better than a traditional neural network directly, but performs worse than some recent knowledge distillation methods.  However, just as in parameter pruning, we show in the last column of Table~\ref{tab:distill_groups} that our SSNs can be combined with prior work to improve performance over using knowledge distillation alone.

\subsection{Analysis of Shapeshifter Networks}
\label{subsec:ssn-analysis}

In this section we compare the components of our SSNs corresponding to the three research questions we raised in the introduction.  Additional analysis on settings such as the number of parameter groups or the number of candidates used to generate weights are in the supplementary. 

Table~\ref{tab:allocation} compares the strategies generating weights from candidates described in Section~\ref{subsec:allocator} when using a single parameter group.  In these experiments we set the number of parameters as the amount are required to implement the largest layer in a network.  For example, the ADAPT-T2I model requires 14M parameters, but its bidirectional GRU accounts for 10M of those parameters, so all SSN variants in this experiment allocate 10M parameters. Comparing to the ``reduced baseline,'' which involves modifying the original model's number and/or size of filters so they have the same number of parameters as our SSNs, we see that the variants of our SNNs perform better, especially on ImageNet where we reduce Error@5 by 3\%.  Across all tasks we can see a trend in learned allocators (Emb, WAvg) performing better than direct methods (RR, Avg).  EmbNet and SimNet even perform better than the fully-parameterized baseline (cf. Table~\ref{tab:groups}) despite their layers operating on different kinds of input features (specifically, vision and language features) with far fewer parameters available.  Also note that prior work in parameter sharing, \eg, SWRN~\cite{savarese2018learning}, can not be applied to the settings in Table~\ref{tab:allocation}, since they require parameter sharing between layers of different types and different operations, or too few parameters.  For example, the WRN-28-10 results use just under 4M parameters, but, as shown in Figure~\ref{fig:param_reduce_compare}(a), SWRN requires at least 12M parameters. %For image classification, our SSNs provide significant parameter savings (requiring 11-28\% the number of the parameters when implemented as a standard neural network) with only a minor impact to task performance.  For example, on ImageNet our approach uses 27.5\% of the weights of the fully-parameterized baseline, but is less than 1\% away from matching its performance.  However, as these classification models also have far more layers than their vision-language counterparts, they are also more likely to benefit from parameter group specialization. As each group will support fewer layers, they may improve performance.

Table~\ref{tab:groups} compares approaches to create parameter groups using the same number of parameters as the original model. We see a small, but largely consistent improvement over using a traditional (baseline) network. Notably, our learned grouping methods (WAvg, Emb) perform on par, and sometimes better than using manual groups. However, our approach can be applied to \emph{any} architecture to create a selected number of parameter groups, making them more flexible than hand-crafted methods. For example, in Table~\ref{tab:upsample}, we see using two groups often helps to improve performance when using very few parameters, but it isn't clear how to effectively create two groups by hand for many networks. 
%Also note that our manual groups for the vision-language models require sharing parameters between layers of different sizes and types, except the WRN results, which use the groups of Savarese~\etal~\cite{savarese2018learning}.  Thus, the "manual" strategy on the image classification task in Table~\ref{tab:groups} represents our implementation of their approach.  We reiterate that a significant benefit of our SSNs learned grouping methods is that they can be applied to \emph{any} network, whereas manual groups from prior work is limited to architectures with identical layers.

In Table~\ref{tab:upsample} we investigate the other new challenge in this work: how to upsample parameters so a large layer operation can be implemented with relatively few parameters. For example, our SSN-WRN-28-10 results use about 0.5M parameters, but the largest layer defined in the network requires just under 4M weights. We find using a simple learned mask to transform parameters performs well on datasets like CIFAR-100, improving Error@1 by 2.5\%.  However, in fully connected (FC) networks using bilinear interpolation performs better.  This is likely because convolutional layers organize parameters into filters that each capture different concepts, but related weights in a FC layer are not well delineated, which forces us to select an arbitrary boundary when using mask upsampling.  Investigating more powerful and efficient parameter upsampling methods, especially for FC layers, is a promising future direction.

%Table~\ref{tab:upsample} along with learning how to create parameter groups automatically, the other new challenge we address in this work is investigating how to upsample parameters so a large layer operation can be performed with few parameters.    We find that the linear method, which uses a fully connected layer to transform weights so they can be reused multiple times tends to overfit.  Using a simple learned mask to transform parameters performs best, improving Error@1 by 2.5\% on CIFAR-100.  Of course, as shown the last column of Table~\ref{tab:upsample}, automatically learning parameter groups to separate layers improves performance even further, even though it can result in additional upsampling after splitting parameters into two parameter stores.











%\subsection{Shapeshifter Networks for Knowledge Distillation}
%\label{subsec:distillation}

%The goal of knowledge distillation is to improve the performance of a small and efficient student by transferring knowledge from a large high performing teacher.  Our SSNs can accomplish a similar feat without using a teacher network by using extra parameters in our student during training, which can be combined statically for inference with no performance loss or increase in memory.

%For example, if a layer requires 2M parameters, but it combines four 2M parameter candidates (8M total) that are not shared with any other layer, its capacity is increased, and the weights can still be precomputed at test time with no performance loss or increase in memory.

%We began by separating each layer into its own parameter group so it would share no parameters with other layers.  We set the number of parameters available to the small student network to be the same as the teacher network in our experimental setup outlined in Table~\ref{tab:distill_setup}.  We began by obtaining a good parameter initialization by training the student SSN to use all of the weights available to it rather than combining multiple candidates using one of the strategies from Section~\ref{subsec:allocator}.  Then, the student is fine-tuned using WAvg since each parameter group contains a single layer and Emb's primary benefit is learning relationships between multiple layers in a parameter group.  Table~\ref{tab:distill_groups} shows that our SSNs obtain competitive performance with other recent knowledge distillation methods, although SSN performs worse than the state-of-the-art.  However, whereas our approach can be thought of as adding additional model flexibility during training, most knowledge transfer methods instead regularize the feature representation learned by the student at multiple points in the network.  As such, we can combine them, resulting in just under 1\% improvement over using knowledge transfer alone as shown in the last column of Table~\ref{tab:distill_groups}.  This helps illustrate the significant potential of SSNs to improve performance and efficiency across a wide variety of neural network architectures and tasks.



==> supp_2_results_std.tex <==
\section{Results with Standard Deviation}
\label{sec:results_std}
The results in our paper are averaged over five runs, except ImageNet which was averaged over three.  In this section we provide standard deviations for our results, which we could not provide in our paper due to space constraints.   This includes bidirectional image-sentence retrieval (Table~\ref{tab:ret_std}), phrase grounding (Table~\ref{tab:ground_std}), image classification (Table~\ref{tab:cls_std}), and knowledge distillation (Table~\ref{tab:distill_std}).  The inclusion of standard deviation helps to solidify the significance of our reported performance gains using SSNs.

\begin{table}[!htbp]
    \centering
    %\setlength{\tabcolsep}{2pt}
    \caption{Bidirectional image-sentence retrieval results with standard deviations from Table 1 and Table 2 from our paper.  Please refer to our paper for number of parameters and groups used for each experiment. Note that  ``Baseline'' refers to using with no parameter sharing, and ``Reduced Baseline'' adjusts the number and/or size of filters of the baseline so they have the same number of parameters as our SSNs.}
    \begin{tabular}{lcccc}
    \toprule
    Architecture & \multicolumn{2}{c}{EmbNet~\cite{Wang_2016_CVPR}} & \multicolumn{2}{c}{ADAPT-T2I~\cite{Wehrmann_2020_AAAI}}\\
    \midrule
    Dataset & F30K~\cite{young2014image} & MSCOCO~\cite{lin2014microsoft} & F30K~\cite{young2014image} & MSCOCO~\cite{lin2014microsoft}\\ 
    \midrule
    \multicolumn{3}{l}{\textbf{Parameter Combiner Comparison}} \\
    \midrule
    Reduced Baseline & 72.8 $\pm$ 0.19 & 80.9 $\pm$ 0.26 & 80.6 $\pm$ 0.15 & 85.2 $\pm$ 0.16\\
    RR & 74.1 $\pm$ 0.25 & 80.8 $\pm$ 0.25 & 81.2 $\pm$ 0.18 & 85.6 $\pm$ 0.18 \\
    Avg & 73.5 $\pm$ 0.21 & 80.9 $\pm$ 0.28 & 80.5 $\pm$ 0.23 & 85.8 $\pm$ 0.21 \\
    WAvg & 74.0 $\pm$ 0.18 & 81.2 $\pm$ 0.22 & 81.6 $\pm$ 0.21 & \textbf{86.2 $\pm$ 0.23}\\
    Emb & \textbf{74.3 $\pm$ 0.27} & \textbf{81.5 $\pm$ 0.32} & \textbf{81.7 $\pm$ 0.19} & 85.9 $\pm$ 0.32\\
    \midrule
        \multicolumn{4}{l}{\textbf{Parameter Bank Grouping Comparison}} \\
        \midrule
        Baseline & 74.1 $\pm$ 0.33 & 81.4 $\pm$ 0.31 & \textbf{83.3 $\pm$ 0.21} & 86.8 $\pm$ 0.17\\
        Single & \textbf{74.4 $\pm$ 0.26} & \textbf{82.1 $\pm$ 0.26} & 82.1 $\pm$ 0.16 & 86.1 $\pm$ 0.19\\
        Random & 74.0 $\pm$ 0.36 & 81.5 $\pm$ 0.25 & 81.9 $\pm$ 0.28 & 86.3 $\pm$ 0.25\\
        Manual & 74.3 $\pm$ 0.24 & 81.7 $\pm$ 0.29 & 82.0 $\pm$ 0.20 & 86.1 $\pm$ 0.21\\
        WAvg & 74.2 $\pm$ 0.23 & 81.7 $\pm$ 0.25 & 82.6 $\pm$ 0.20 & 86.4 $\pm$ 0.17\\
        Emb & 74.3 $\pm$ 0.14 & 81.9 $\pm$ 0.30 & 82.9 $\pm$ 0.22 & \textbf{87.0 $\pm$ 0.23}\\
        \bottomrule
    \end{tabular}
    \label{tab:ret_std}
\end{table}

\begin{table}[!htbp]
    \centering
    %\setlength{\tabcolsep}{2pt}
    \caption{Phrase grounding results with standard deviations from Table 1 and Table 2 from our paper.  Please refer to our paper for number of parameters and groups used for each experiment. Note that  ``Baseline'' refers to using no parameter sharing, and ``Reduced Baseline'' adjusts the number and/or size of filters of the baseline so they have the same number of parameters as our SSNs.}
    \begin{tabular}{lcc}
    \toprule
    Architecture & \multicolumn{2}{c}{SimNet~\cite{wang2018learning}} \\
    \midrule
    Dataset & F30K Entities~\cite{flickrentitiesijcv} & ReferIt~\cite{kazemzadeh-EtAl:2014:EMNLP2014}\\ 
    \midrule
    \multicolumn{3}{l}{\textbf{Parameter Combiner Comparison}} \\
    \midrule
    Reduced Baseline & 71.1 $\pm$ 0.28 & 59.4 $\pm$ 0.49\\
    RR & 72.3 $\pm$ 0.28 & \textbf{60.5 $\pm$ 0.53}\\
    Avg & 72.1 $\pm$ 0.31 & 60.2 $\pm$ 0.53\\
    WAvg & 72.3 $\pm$ 0.25 & \textbf{60.5 $\pm$ 0.48}\\
    Emb & \textbf{72.5 $\pm$ 0.30} & 60.4 $\pm$ 0.52\\
    \midrule
        \multicolumn{3}{l}{\textbf{Parameter Bank Grouping Comparison}} \\
        \midrule
        Baseline & 71.7 $\pm$ 0.26 & \textbf{61.1 $\pm$ 0.39}\\
        Single & 71.4 $\pm$ 0.33 & 60.9 $\pm$ 0.56\\
        Random & 71.8 $\pm$ 0.43 & 60.0 $\pm$ 0.57\\
        Manual & \textbf{72.4 $\pm$ 0.29} & 60.2 $\pm$ 0.49\\
        WAvg & 72.2 $\pm$ 0.34 & 61.0 $\pm$ 0.43\\
        Emb & 72.1 $\pm$ 0.28 & 60.5 $\pm$ 0.57\\
        \bottomrule
    \end{tabular}
    \label{tab:ground_std}
\end{table}

\begin{table}[!htbp]
    \centering
    %\setlength{\tabcolsep}{2pt}
    \caption{Image classification results with standard deviations from Table 1 and Table 2 from our paper.  Please refer to our paper for number of parameters and groups in each experiment. Note that  ``Baseline'' refers to using no parameter sharing, and ``Reduced Baseline'' adjusts the number and/or size of filters of the baseline so they have the same number of parameters as our SSNs.}
    \begin{tabular}{lccc}
    \toprule
    Architecture & \multicolumn{2}{c}{WRN-28-10~\cite{Zagoruyko2016WRN}} & WRN-50-2~\cite{Zagoruyko2016WRN}\\
    \midrule
    Dataset & CIFAR-10~\cite{cifar} & CIFAR-100~\cite{cifar} & ImageNet~\cite{deng2009imagenet}\\ \midrule
    \multicolumn{3}{l}{\textbf{Parameter Combiner Comparison}} \\
    \midrule
    Reduced Baseline & 4.22 $\pm$ 0.16 & 22.34 $\pm$ 0.12 & 10.08 $\pm$ 0.02\\
    RR & 4.09 $\pm$ 0.34 & 21.91 $\pm$ 0.24 & \textbf{6.69 $\pm$ 0.08}\\
    Avg & 4.19 $\pm$ 0.11 & 22.78 $\pm$ 0.29 & 7.61 $\pm$ 0.07\\
    WAvg & 4.00 $\pm$ 0.08 & \textbf{21.78 $\pm$ 0.26} & 7.38 $\pm$ 0.02\\
    Emb & \textbf{3.84 $\pm$ 0.13} & 21.92 $\pm$ 0.30 & \textbf{6.69 $\pm$ 0.11}\\
    \midrule
        \multicolumn{4}{l}{\textbf{Parameter Bank Grouping Comparison}} \\
        \midrule
        Baseline & 3.57 $\pm$ 0.19 & 19.44 $\pm$ 0.21 & 5.84 $\pm$ 0.06\\
        Single & 3.71 $\pm$ 0.17 & 19.99 $\pm$ 0.22 & 6.18 $\pm$ 0.05\\
        Random & 3.63 $\pm$ 0.11 & 20.36 $\pm$ 0.50 & 5.91 $\pm$ 0.08\\
        Manual & \textbf{3.38 $\pm$ 0.14} & 19.29 $\pm$ 0.26 & \textbf{5.82 $\pm$ 0.01}\\
        WAvg & 3.51 $\pm$ 0.11 & 19.47 $\pm$ 0.30 & 5.86 $\pm$ 0.06\\
        Emb & 3.42 $\pm$ 0.06 & \textbf{19.24 $\pm$ 0.29} & 5.96 $\pm$ 0.06\\
        \bottomrule
    \end{tabular}
    \label{tab:cls_std}
\end{table}


\begin{table}[!htbp]
    \centering
    \caption{Experimental setup for our knowledge distillation experiments reported in Table~\ref{tab:distill_std}.}
    \begin{tabular}{cccccc}
    \toprule
    Experiment & Teacher & \#Params (M) & Student  & \#Params (M) & Dataset\\
    \midrule
        (a) & WRN-28-4 & 5.87 & WRN-28-2 & 1.47 & CIFAR-100\\
        (b) & WRN-28-4 & 5.87 & WRN-16-2 & 0.70 & CIFAR-100\\
    \bottomrule
    \end{tabular}
    \label{tab:distill_setup}
\end{table}

\begin{table}[!htbp]
    \centering
    \caption{Knowledge distillation results with standard deviation on CIFAR-100 using teacher/student setup in Table~\ref{tab:distill_setup}.  Note our SSNs only use a teacher network when combined with OD~\cite{Heo_2019_ICCV}.  See Section 4.3 of our paper for discussion.}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{cccccccccccc}
    \toprule
    Experiment & Teacher & Baseline & AT~\cite{Zagoruyko2017AT} & Jacobian~\cite{SrinivasJacobianICML2018} & FT~\cite{kimFactorTransfer2018} & AB~\cite{ABdistill} & OD~\cite{Heo_2019_ICCV} & SSN (ours) & SSN+OD\\
    \midrule
        (a) & 21.09 & 24.88 & 23.80 & 23.70 & 23.41 & 23.19 & 21.98 & 23.62 $\pm$ 0.13 & \textbf{21.21 $\pm$ 0.21}\\
        (b) & 21.09 & 27.32 & 26.56 & 26.71 & 25.91 & 26.02 & 24.08 & 26.53 $\pm$ 0.15 & \textbf{23.30 $\pm$ 0.19}\\
    \bottomrule
    \end{tabular}
    \label{tab:distill_std}
\end{table}

%\clearpage
